Performant near-term quantum combinatorial optimization

Combinatorial optimization is a promising application for near-term quantum computers, however, identifying performant algorithms suited to noisy quantum hardware remains as an important goal to potentially realizing quantum computational advantages. To address this we present a variational quantum algorithm for solving combinatorial optimization problems with linear-depth circuits. Our algorithm uses an ansatz composed of Hamiltonian generators designed to control each term in the target combinatorial function, along with parameter updates following a modified version of quantum imaginary time evolution. We evaluate this ansatz in numerical simulations that target solutions to the MAXCUT problem. The state evolution is shown to closely mimic imaginary time evolution, and its optimal-solution convergence is further improved using adaptive transformations of the classical Hamiltonian spectrum. With these innovations, the algorithm consistently converges to optimal solutions, with interesting highly-entangled dynamics along the way. We further demonstrate the success of this approach by performing optimization of a truncated version of our ansatz with up to 32 qubits in a trapped-ion quantum computer, using measurements from the quantum computer to train the ansatz and prepare optimal solutions with high fidelity in the majority of cases we consider. The success of these large-scale quantum circuit optimizations, in the presence of realistic hardware constraints and without error mitigation, mark significant progress on the path towards solving combinatorial problems using quantum computers. We conclude our performant and resource-minimal approach is a promising candidate for potential quantum computational advantages.

==> Binary_opt/supp_natcom.tex <==
\pagebreak
\widetext
\begin{center}
\textbf{\large Supplemental Materials: Performant near-term quantum combinatorial optimization}
\end{center}
%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{1}
\makeatletter
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
%\renewcommand{\citenumfont}[1]{S#1}
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%




\section{Ansatz}
In pursuit of a solution of the binary optimization problem, we perform an analysis of the QAOA ansatz,  
\begin{align}
\ket{\vec{\theta},\vec{\gamma}}_p = \prod_{j=0}^{p}\exp(-i\gamma_j H_m)\exp(-i\theta_j H_c)\ket{+}^\otimes ,
\end{align}
where $H_m$ is the standard mixing Hamiltonian and $H_c$ is the cost Hamiltonian with an eigenspectrum $H_c \ket{\bm z} = C(\bm z)\ket{\bm z}$ that contains the set of classical solution values 
\begin{align}
H_m = -\sum_{j \in V}X_j \\
H_c = \sum_{j,k \in E}\omega_{jk}Z_j Z_k = \sum_\alpha \lambda_\alpha P_\alpha \,.
\end{align}

In the limit as $p \rightarrow \infty$, and with appropriately chosen $\vec{\theta}$ and $\vec{\gamma}$, the QAOA ansatz yields adiabatic evolution from the ground state $\ket{+}^{\otimes n}$ of $H_m$ to the optimal-solution ground state $\ket{\bm z_\mathrm{opt}}$ of $H_c$. At finite $p$ that are implementable on current quantum computers, QAOA has been shown to be successful at approximating $\ket{\bm z_\mathrm{opt}}$ by variationally optimizing the parameters $p$. Analyzing the QAOA/adiabatic ansatz by combining the two sequential applications of a single layer under its equivalent single exponential is illustrative.

The leading order term after the sum of the driving and mixing Hamiltonians is their single commutator
\begin{align}
-\frac{\gamma_j*\theta_j}{2}[H_m,H_c] = -\frac{i\gamma_j*\theta_j}{2}\sum_{k,l \in E}\omega_{kl}(Y_k Z_l+Z_k Y_l) \,.
\end{align}
Previous work in accelerating convergence within QAOA found these are precisely the terms most important for accelerating convergence \cite{chandarana2022,Zhu2022}.  

Is it clear from the following relation
\begin{align}
\exp(\frac{i\pi ZY}{2})
\left\{
    \begin{array}{lr}
        \ket{00}\pm \ket{11} \\
        \ket{01}\pm \ket{10} 
    \end{array}
\right\} = 
\left\{
    \begin{array}{lr}
        \mp \ket{01}\mp \ket{10} \\
         \quad   \ket{00}\pm \ket{11} 
    \end{array}
\right\}  
\end{align}
that $ZY$ rotations exactly rotate norm between the $\pm 1$ sector of $ZZ$ terms of the Hamiltonian.  Based on these findings, we employ a parameterized ansatz of the form 
\begin{align}
\ket{\Psi(\theta)} = \prod_{j = \{(r,q) : r<q\} \in |V|}\exp(i\theta_{j}Z_rY_q)\ket{+}^\otimes
\end{align} 
where $j$ indexes all unique pairs of vertices.  
The ordering is important for robust convergence, so we introduce the quantity 
\begin{align}
\rho_j = \sum_{k \in E}|\omega_{jk}|
\end{align}
which represents the relative importance of each vertex in the overall $H_c$. Thus in this work, we order the $ZY$ rotations in the ansatz by their corresponding size in $\rho$.  For a vertex set $|V|$ indexed now by their order in $\rho$, the ansatz exploited in this work has an explicit form
\begin{align}
\ket{\Psi(\theta)} = \exp(i\theta_{j}Z_{N-1}Y_{N})\ldots \exp(i\theta_{j}Z_0Y_2)\exp(i\theta_{j}Z_0Y_1)\ket{+}^\otimes\,.
\end{align} 
\begin{figure*}[ht]
    \centering
    % \includegraphics[width=\columnwidth]{HiddenInversesQSCOUT/work_flow_redo.PNG}
    %\includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_graphsize16_plot.png}
    %\includegraphics[width=.85\columnwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log.png}
    %\includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log_combined.png}  
    \includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log_combined_only3_rr.png}  
    \caption{Average error convergence for 100 random instances of (a) 3 regular, (b) NWS, and (c) SK graphs with 16 vertices and relaxed rounding performed. The orange line is VAR-IT, the green line is (\ref{eq:ansatz_form}) optimized with ADAM, and the purple line shows the optimized error from 8-layer QAOA [from \cite{dupont2024,dupontpersonal}]. }  
    \label{fig:convergence_rr}
\end{figure*}
\section{Problem types}
The different problem types explored in this work are dictated by the $\omega_{ij}$ between vertices, commonly referred to as the adjacency matrix.  All graphs in this work are generated by the Python package NetworkX \cite{networkx}.

{\it Sherrington-Kirkpatrick (SK)} -- The SK model in this work is defined as the fully connected graph type, with $\omega_{ij}$ chosen between $\pm1$ chosen with equal probability. 

{\it Newman-Watts-Strogatz small-world graphs (NWS)} -- In order to create models of this type, vertices of a ring graph are connected with its $k$ nearest neighbors.  In this work, $k=4$.  Afterwards, for each resulting edge (i,j), in the ring with connections to k nearest neighbors, add a new edge (i,l) with probability $p$, in this work $p=0.5$, to a randomly-chosen vertex $l$. Then $\omega_{ij}$ are assigned randomly in the interval $(0,1]$.

{\it Random 3 Regular (3Reg)} -- This model arises from graphs where each vertex is connected to three other vertices randomly.  $\omega_{ij}$ are all assigned a uniform value of 1 in this case.

\section{Relaxed Rounding}
In \cite{dupont2024}, the authors introduced a quantum analogue of the classical relax and round method.  They showed that it can easily be used to augment wavefunction methods like QAOA, and always improves the approximation ratio. It relies on the establishing the correlation matrix $\chi_{ij}$, defined as 
\begin{align}
\chi_{ij} = (\delta_{ij}-1)\langle Z_iZ_j\rangle \,.
\end{align}
Then $\chi$ can be diagonalized classically to yield its eigenvectors $\{\alpha_\nu \in \mathbb{R}^N\}$.  These can be translated to their closest bitstrings by rounding $\{z_\nu \leftarrow sign(\alpha_\nu) \in {\pm 1}^N\}$. Then the $z_\nu$ which minimizes the $C(z)$ is chosen as the outcome of this quantum,relax, and round procedure.  We apply this procedure at each iteration of our optimization procedure and report the findings in Fig. \ref{fig:convergence_rr}.



\section{Further Numerical Results}
In numerical results section of this work, we presented the error of the approximation ratio when using our VAR-IT method for optimization of Eq. \ref{eq:ansatz_form}, and the ADAM optimizer.  

\begin{figure}[h]
    \centering
    % \includegraphics[width=\columnwidth]{HiddenInversesQSCOUT/work_flow_redo.PNG}
    %\includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_graphsize16_plot.png}
    %\includegraphics[width=.85\columnwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log.png}
    %\includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log_combined.png}  
    \includegraphics[width=\columnwidth]{Binary_opt/figs/new_iterations.png}  
    \caption{ Average iterations required as a function of graph size. }  
    \label{fig:iterationtoconv}
\end{figure}
\begin{figure*}[!b]
    \centering
    % \includegraphics[width=\columnwidth]{HiddenInversesQSCOUT/work_flow_redo.PNG}
    %\includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_graphsize16_plot.png}
    %\includegraphics[width=.85\columnwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log.png}
    %\includegraphics[width=\textwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_log_combined.png}  
    \includegraphics[width=.9\textwidth]{Binary_opt/figs/convergence_3reg_nws_sk_graphsize16_failure.png}  
    \caption{Fraction of instances with $<1\%$ norm on optimal solutions after 100 iterations. }  
    \label{fig:failure}
\end{figure*}
In addition to the VAR-IT method always converging to an optimal solution, Fig. \ref{fig:iterationtoconv} demonstrates that for the sizes explored in this work, the iterations required to reach convergence for all three problem types explored in this work appear to be scaling linearly in problem size.  Additionally, Fig. \ref{fig:failure} shows that an ansatz optimized with ADAM will yield increasing failures as problem size grows, while there does not appear to be any such signature with the VAR-IT optimization procedure.
